Charon: An Analysis Framework for Rust

With the explosion in popularity of the Rust programming language, a wealth of tools have recently been developed to analyze, verify, and test Rust programs. Alas, the Rust ecosystem remains relatively young, meaning that every one of these tools has had to re-implement difficult, time-consuming machinery to interface with the Rust compiler and its cargo build system, to hook into the Rust compiler's internal representation, and to expose an abstract syntax tree (AST) that is suitable for analysis rather than optimized for efficiency. We address this missing building block of the Rust ecosystem, and propose Charon, an analysis framework for Rust. Charon acts as a swiss-army knife for analyzing Rust programs, and deals with all of the tedium above, providing clients with a clean, stable AST that can serve as the foundation of many analyses. We demonstrate the usefulness of Charon through a series of case studies, ranging from a Rust verification framework (Aeneas), a compiler from Rust to C (Eurydice), and a novel taint-checker for cryptographic code. To drive the point home, we also re-implement a popular existing analysis (Rudra), and show that it can be replicated by leveraging the Charon framework.

==> Makefile <==
.SUFFIXES: .dvi .ps

PAPER = paper
LATEX = latex
PDFLATEX = pdflatex
TEXFILES = *.tex
BIBFILE = cited.bib conferences.bib


default: $(PAPER).pdf

$(PAPER).pdf: $(TEXFILES) $(BIBFILE)
	latexmk -pdf -shell-escape $(PAPER).tex

pvc: $(TEXFILES) $(BIBFILE)
	latexmk -halt-on-error -pvc -pdf -shell-escape $(PAPER).tex

final:	$(PAPER).pdf
	cp $(PAPER).pdf final.pdf

clean:
	rm -fr *.ps *.bcf *.run.xml *.fls *.fdb_latexmk *.dvi *.aux *.bbl *.blg *.log *.out *.toc $(PAPER).pdf *~

# To submit online
.PHONY: sources
sources:
	rm -rf sources
	mkdir -p sources
	cp llncs.cls sources/
	cp splncs04.bst sources/
	cp figure1.pdf sources/
	cp 1-available.pdf sources/
	cp 2-functional.pdf sources/
	cp 3-reusable.pdf sources/
	cp paper.bbl sources/
	cp cited.bib sources/
	cp conferences.bib sources/
	cp paper.tex sources/
	cp -r _minted-paper sources/
	cp Makefile sources/
	rm -rf sources.zip && zip -r sources sources

.PHONY: sources.zip
sources.zip:
	rm -rf sources.zip && zip -r sources sources

#	sed -i 's/%\\usepackage\[frozencache=true\]{minted}/\\usepackage\[frozencache=true\]{minted}/' online/paper.tex
#	sed -i 's/\\usepackage\[frozencache=false,finalizecache=true\]{minted}//' online/paper.tex

